A second order local minimality criterion for the triple junction singularity of the Mumford-Shah functional

This paper is the first part of an ongoing project aimed at providing a local minimality criterion, based on a second variation approach, for the triple point configurations of the Mumford-Shah functional.

==> Commands.tex <==
%Spaces

\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\M}{\mathbb M}


%Math symbols

\newcommand{\tr}{{\rm trace\,}}
\renewcommand{\div}{{\rm div}}
\newcommand{\dist}{{\rm dist\,}}
\newcommand{\supp}{{\rm supp\,}}
\newcommand{\cap}{{\rm cap}}


%Measures

\newcommand{\l}{{\mathcal L}}
\newcommand{\hn}{{\mathcal{H}}^N}
\newcommand{\hno}{{\mathcal H}^{N-1}}
\newcommand{\hnt}{{\mathcal H}^{N-2}}
\newcommand{\ho}{{\mathcal H}^{1}}
\newcommand{\hz}{{\mathcal H}^{0}}


%Abbreviations

\newcommand{\wto}{\rightharpoonup}
\newcommand{\meno}{\!\setminus\!}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\e}{\varepsilon}
\newcommand{\p}{\varphi}


%Functionals

\newcommand{\f}{\mathcal{F}}
\newcommand{\p}{\mathcal{P}}
\newcommand{\nl}{\mathcal{NL}}
\newcommand{\ms}{\mathcal{MS}}


%Other stuff

\newcommand{\mloc}{m_{\rm loc}}
\newcommand{\mglob}{m_{\rm glob}}
